A PTAS for Minimizing Weighted Flow Time on a Single Machine

An important objective in scheduling literature is to minimize the sum of weighted flow times. We are given a set of jobs where each job is characterized by a release time, a processing time, and a weight. Our goal is to find a preemptive schedule on a single machine that minimizes the sum of the weighted flow times of the jobs, where the flow time of a job is the time between its completion time and its release time. The currently best known polynomial time algorithm for the problem is a (2+eps)-approximation by Rohwedder and Wiese [STOC 2021] which builds on the prior break-through result by Batra, Garg, and Kumar [FOCS 2018] who found the first pseudo-polynomial time constant factor approximation algorithm for the problem, and on the result by Feige, Kulkarni, and Li [SODA 2019] who turned the latter into a polynomial time algorithm. However, it remains open whether the problem admits a PTAS. We answer this question in the affirmative and present a polynomial time (1+eps)-approximation algorithm for weighted flow time on a single machine. We rely on a reduction of the problem to a geometric covering problem, which was introduced in the mentioned (2+eps)-approximation algorithm, losing a factor 1+eps in the approximation ratio. However, unlike that algorithm, we solve the resulting instances of this problem exactly, rather than losing a factor 2+eps. Key for this is to identify and exploit structural properties of instances of the geometric covering problem which arise in the reduction from weighted flow time.

==> fig-base-small.tex <==
  \node at (9.75, 8) {\dots};
  \node at (7, 9.25) {$\vdots$};

  \def\y{10 - 12 * \dy}
  
  \foreach \i in {18,...,39} {
  \draw (\i * 0.5 / 4, \y) rectangle (\i * 0.5 / 4 + 0.5 / 4, \y + \dy);
  }

  \draw (5, \y) rectangle (5.5, \y + \dy);
  \draw (5.5, \y) rectangle (6, \y + \dy);
  \draw (6, \y) rectangle (6.5, \y + \dy);
  \draw (6.5, \y) rectangle (7, \y + \dy);
  \draw (7, \y) rectangle (7.5, \y + \dy);
  \draw (7.5, \y) rectangle (9, \y + \dy);
  \draw (8, \y) rectangle (8.5, \y + \dy);
  \draw (8.5, \y) rectangle (9, \y + \dy);


  \def\y{10 - 13 * \dy}

  \foreach \i in {35,...,55} {
  \draw (\i * 0.5 / 4, \y) rectangle (\i * 0.5 / 4 + 0.5 / 4, \y + \dy);
  }

  \draw (7, \y) rectangle (7.5, \y + \dy);
  \draw (7.5, \y) rectangle (8, \y + \dy);
  \draw (8, \y) rectangle (8.5, \y + \dy);
  \draw (8.5, \y) rectangle (9, \y + \dy);


  \def\y{10 - 14 * \dy}
  
  \foreach \i in {40,...,55} {
  \draw (\i * 0.5 / 4, \y) rectangle (\i * 0.5 / 4 + 0.5 / 4, \y + \dy);
  }

  \draw (7, \y) rectangle (7.5, \y + \dy);
  \draw (7.5, \y) rectangle (8, \y + \dy);
  \draw (8, \y) rectangle (8.5, \y + \dy);
  \draw (8.5, \y) rectangle (9, \y + \dy);

  \def\y{10 - 15 * \dy}
  
  \foreach \i in {50,...,71} {
  \draw (\i * 0.5 / 4, \y) rectangle (\i * 0.5 / 4 + 0.5 / 4, \y + \dy);
  }

  \def\y{10 - 16 * \dy}
  
  \foreach \i in {51,...,71} {
  \draw (\i * 0.5 / 4, \y) rectangle (\i * 0.5 / 4 + 0.5 / 4, \y + \dy);
  }
  \def\y{10 - 17 * \dy}
  
  \foreach \i in {60,...,71} {
  \draw (\i * 0.5 / 4, \y) rectangle (\i * 0.5 / 4 + 0.5 / 4, \y + \dy);
  }

==> fig-base.tex <==

  \node at (-0.5, 9.75) {\dots};
  \node at (14, 9.75) {\dots};
  \node at (14, 7.75) {\dots};
  \def\y{10}
%  \node at (-0.5, \y + 0.5 * \dy) {\dots};
  \draw (0, \y) rectangle (13.5, \y + \dy);

  \def\y{10 - \dy}
%  \node at (-0.5, \y + 0.5 * \dy) {\dots};
  \draw (0, \y) rectangle (13.5, \y + \dy);

  \def\y{10 - 2 * \dy}
%  \node at (-0.5, \y + 0.5 * \dy) {\dots};

  \draw (0, \y) rectangle (4.5, \y + \dy);
  \draw (4.5, \y) rectangle (9, \y + \dy);
  \draw (9, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (0 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 3 * \dy}
%  \node at (-0.5, \y + 0.5 * \dy) {\dots};

  \draw (0, \y) rectangle (4.5, \y + \dy);
  \draw (4.5, \y) rectangle (9, \y + \dy);
  \draw (9, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (0 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 3 * \dy}
%  \node at (-0.5, \y + 0.5 * \dy) {\dots};

  \draw (0, \y) rectangle (1.5, \y + \dy);
  \draw (1.5, \y) rectangle (3, \y + \dy);
  \draw (3, \y) rectangle (4.5, \y + \dy);
%  \fill[white] (0 + 0.1, \y + 0.7 * \dy) rectangle (4.5 - 0.1, \y + 0.3 * \dy);

  \draw (4.5, \y) rectangle (6, \y + \dy);
  \draw (6, \y) rectangle (7.5, \y + \dy);
  \draw (7.5, \y) rectangle (9, \y + \dy);

  \draw (9, \y) rectangle (10.5, \y + \dy);
  \draw (10.5, \y) rectangle (12, \y + \dy);
  \draw (12, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (4.5 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 4 * \dy}

  \draw (0 * 0.5 / 3, \y) rectangle (1 * 0.5 / 3, \y + \dy);
  \draw (1 * 0.5 / 3, \y) rectangle (2 * 0.5 / 3, \y + \dy);
  \draw (2 * 0.5 / 3, \y) rectangle (3 * 0.5 / 3, \y + \dy);
  \draw (3 * 0.5 / 3, \y) rectangle (4 * 0.5 / 3, \y + \dy);
  \draw (4 * 0.5 / 3, \y) rectangle (5 * 0.5 / 3, \y + \dy);
  \draw (5 * 0.5 / 3, \y) rectangle (6 * 0.5 / 3, \y + \dy);
  \draw (6 * 0.5 / 3, \y) rectangle (7 * 0.5 / 3, \y + \dy);
  \draw (7 * 0.5 / 3, \y) rectangle (8 * 0.5 / 3, \y + \dy);
  \draw (8 * 0.5 / 3, \y) rectangle (9 * 0.5 / 3, \y + \dy);

  \draw (1.5, \y) rectangle (2, \y + \dy);
  \draw (2, \y) rectangle (2.5, \y + \dy);
  \draw (2.5, \y) rectangle (3, \y + \dy);

  \draw (3, \y) rectangle (3.5, \y + \dy);
  \draw (3.5, \y) rectangle (4, \y + \dy);
  \draw (4, \y) rectangle (4.5, \y + \dy);
%  \fill[white] (1.5 + 0.1, \y + 0.7 * \dy) rectangle (4.5 - 0.1, \y + 0.3 * \dy);

  \draw (4.5, \y) rectangle (6, \y + \dy);
  \draw (6, \y) rectangle (7.5, \y + \dy);
  \draw (7.5, \y) rectangle (9, \y + \dy);

  \draw (9, \y) rectangle (10.5, \y + \dy);
  \draw (10.5, \y) rectangle (12, \y + \dy);
  \draw (12, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (4.5 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 5 * \dy}

  \draw (5 * 0.5 / 3, \y) rectangle (6 * 0.5 / 3, \y + \dy);
  \draw (6 * 0.5 / 3, \y) rectangle (7 * 0.5 / 3, \y + \dy);
  \draw (7 * 0.5 / 3, \y) rectangle (8 * 0.5 / 3, \y + \dy);
  \draw (8 * 0.5 / 3, \y) rectangle (9 * 0.5 / 3, \y + \dy);

  \draw (1.5, \y) rectangle (2, \y + \dy);

%  \draw[thick, red] (1, \y) rectangle (1.5, \y + \dy);

  \draw (2, \y) rectangle (2.5, \y + \dy);
  \draw (2.5, \y) rectangle (3, \y + \dy);
%  \fill[white] (1.5 + 0.1, \y + 0.7 * \dy) rectangle (3 - 0.1, \y + 0.3 * \dy);

  \draw (3, \y) rectangle (3.5, \y + \dy);
  \draw (3.5, \y) rectangle (4, \y + \dy);
  \draw (4, \y) rectangle (4.5, \y + \dy);
%  \fill[white] (3 + 0.1, \y + 0.7 * \dy) rectangle (4.5 - 0.1, \y + 0.3 * \dy);

  \draw (4.5, \y) rectangle (6, \y + \dy);
  \draw (6, \y) rectangle (7.5, \y + \dy);
  \draw (7.5, \y) rectangle (9, \y + \dy);

  \draw (9, \y) rectangle (10.5, \y + \dy);
  \draw (10.5, \y) rectangle (12, \y + \dy);
  \draw (12, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (4.5 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);
  
%  \fill[pattern color=red, pattern=north west lines] (7.5, \y) rectangle (9, \y + \dy);

  \def\y{10 - 6 * \dy}

  \draw (10 * 0.5 / 3, \y) rectangle (11 * 0.5 / 3, \y + \dy);
  \draw (11 * 0.5 / 3, \y) rectangle (12 * 0.5 / 3, \y + \dy);
  \draw (12 * 0.5 / 3, \y) rectangle (13 * 0.5 / 3, \y + \dy);
  \draw (13 * 0.5 / 3, \y) rectangle (14 * 0.5 / 3, \y + \dy);
  \draw (14 * 0.5 / 3, \y) rectangle (15 * 0.5 / 3, \y + \dy);
  \draw (15 * 0.5 / 3, \y) rectangle (16 * 0.5 / 3, \y + \dy);
  \draw (16 * 0.5 / 3, \y) rectangle (17 * 0.5 / 3, \y + \dy);
  \draw (17 * 0.5 / 3, \y) rectangle (18 * 0.5 / 3, \y + \dy);
  
  \draw (3, \y) rectangle (3.5, \y + \dy);
  \draw (3.5, \y) rectangle (4, \y + \dy);
  \draw (4, \y) rectangle (4.5, \y + \dy);
%  \fill[white] (3 + 0.1, \y + 0.7 * \dy) rectangle (4.5 - 0.1, \y + 0.3 * \dy);

  \draw (4.5, \y) rectangle (6, \y + \dy);
  \draw (6, \y) rectangle (7.5, \y + \dy);
  \draw (7.5, \y) rectangle (9, \y + \dy);

  \draw (9, \y) rectangle (10.5, \y + \dy);
  \draw (10.5, \y) rectangle (12, \y + \dy);
  \draw (12, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (9 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 7 * \dy}

  \draw (20 * 0.5 / 3, \y) rectangle (21 * 0.5 / 3, \y + \dy);
  \draw (21 * 0.5 / 3, \y) rectangle (22 * 0.5 / 3, \y + \dy);
  \draw (22 * 0.5 / 3, \y) rectangle (23 * 0.5 / 3, \y + \dy);
  \draw (23 * 0.5 / 3, \y) rectangle (24 * 0.5 / 3, \y + \dy);
  \draw (24 * 0.5 / 3, \y) rectangle (25 * 0.5 / 3, \y + \dy);
  \draw (25 * 0.5 / 3, \y) rectangle (26 * 0.5 / 3, \y + \dy);
  \draw (26 * 0.5 / 3, \y) rectangle (27 * 0.5 / 3, \y + \dy);

  \draw (4.5, \y) rectangle (5, \y + \dy);
  \draw (5, \y) rectangle (5.5, \y + \dy);
  \draw (5.5, \y) rectangle (6, \y + \dy);
  \draw (6, \y) rectangle (6.5, \y + \dy);
  \draw (6.5, \y) rectangle (7, \y + \dy);
  \draw (7, \y) rectangle (7.5, \y + \dy);
  \draw (7.5, \y) rectangle (9, \y + \dy);
  \draw (8, \y) rectangle (8.5, \y + \dy);
  \draw (8.5, \y) rectangle (9, \y + \dy);
%  \fill[white] (4.5 + 0.1, \y + 0.7 * \dy) rectangle (9 - 0.1, \y + 0.3 * \dy);
%  \fill[pattern color=red, pattern=north west lines] (8, \y) rectangle (8.5, \y + \dy);

  \draw (9, \y) rectangle (10.5, \y + \dy);
  \draw (10.5, \y) rectangle (12, \y + \dy);
  \draw (12, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (9 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 8 * 0.5/3}
  \draw (21 * 0.5 / 3, \y) rectangle (22 * 0.5 / 3, \y + \dy);
  \draw (22 * 0.5 / 3, \y) rectangle (23 * 0.5 / 3, \y + \dy);
  \draw (23 * 0.5 / 3, \y) rectangle (24 * 0.5 / 3, \y + \dy);
  \draw (24 * 0.5 / 3, \y) rectangle (25 * 0.5 / 3, \y + \dy);
  \draw (25 * 0.5 / 3, \y) rectangle (26 * 0.5 / 3, \y + \dy);
  \draw (26 * 0.5 / 3, \y) rectangle (27 * 0.5 / 3, \y + \dy);

  \draw (4.5, \y) rectangle (5, \y + \dy);
  \draw (5, \y) rectangle (5.5, \y + \dy);
  \draw (5.5, \y) rectangle (6, \y + \dy);
  \draw (6, \y) rectangle (6.5, \y + \dy);
  \draw (6.5, \y) rectangle (7, \y + \dy);
  \draw (7, \y) rectangle (7.5, \y + \dy);
  \draw (7.5, \y) rectangle (9, \y + \dy);
  \draw (8, \y) rectangle (8.5, \y + \dy);
  \draw (8.5, \y) rectangle (9, \y + \dy);
%  \fill[white] (4.5 + 0.1, \y + 0.7 * \dy) rectangle (9 - 0.1, \y + 0.3 * \dy);
%  \fill[pattern color=red, pattern=north west lines] (8, \y) rectangle (8.5, \y + \dy);

  \draw (9, \y) rectangle (10.5, \y + \dy);
  \draw (10.5, \y) rectangle (12, \y + \dy);
  \draw (12, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (9 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 9 * 0.5/3}

  \draw (22 * 0.5 / 3, \y) rectangle (23 * 0.5 / 3, \y + \dy);
  \draw (23 * 0.5 / 3, \y) rectangle (24 * 0.5 / 3, \y + \dy);
  \draw (24 * 0.5 / 3, \y) rectangle (25 * 0.5 / 3, \y + \dy);
  \draw (25 * 0.5 / 3, \y) rectangle (26 * 0.5 / 3, \y + \dy);
  \draw (26 * 0.5 / 3, \y) rectangle (27 * 0.5 / 3, \y + \dy);

  \draw (4.5, \y) rectangle (5, \y + \dy);
  \draw (5, \y) rectangle (5.5, \y + \dy);
  \draw (5.5, \y) rectangle (6, \y + \dy);
%  \fill[white] (4.5 + 0.1, \y + 0.7 * \dy) rectangle (6 - 0.1, \y + 0.3 * \dy);

  \draw (6, \y) rectangle (6.5, \y + \dy);
  \draw (6.5, \y) rectangle (7, \y + \dy);
  \draw (7, \y) rectangle (7.5, \y + \dy);
  \draw (7.5, \y) rectangle (9, \y + \dy);
  \draw (8, \y) rectangle (8.5, \y + \dy);
  \draw (8.5, \y) rectangle (9, \y + \dy);
%  \fill[white] (6 + 0.1, \y + 0.7 * \dy) rectangle (9 - 0.1, \y + 0.3 * \dy);
%  \fill[pattern color=red, pattern=north west lines] (8, \y) rectangle (8.5, \y + \dy);

  \draw (9, \y) rectangle (10.5, \y + \dy);
  \draw (10.5, \y) rectangle (12, \y + \dy);
  \draw (12, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (9 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 10 * 0.5/3}
  
  \draw (25 * 0.5 / 3, \y) rectangle (26 * 0.5 / 3, \y + \dy);
  \draw (26 * 0.5 / 3, \y) rectangle (27 * 0.5 / 3, \y + \dy);
  \draw (27 * 0.5 / 3, \y) rectangle (28 * 0.5 / 3, \y + \dy);
  \draw (28 * 0.5 / 3, \y) rectangle (29 * 0.5 / 3, \y + \dy);
  \draw (29 * 0.5 / 3, \y) rectangle (30 * 0.5 / 3, \y + \dy);
  \draw (30 * 0.5 / 3, \y) rectangle (31 * 0.5 / 3, \y + \dy);
  \draw (31 * 0.5 / 3, \y) rectangle (32 * 0.5 / 3, \y + \dy);
  \draw (32 * 0.5 / 3, \y) rectangle (33 * 0.5 / 3, \y + \dy);
  \draw (33 * 0.5 / 3, \y) rectangle (34 * 0.5 / 3, \y + \dy);
  \draw (34 * 0.5 / 3, \y) rectangle (35 * 0.5 / 3, \y + \dy);
  \draw (35 * 0.5 / 3, \y) rectangle (36 * 0.5 / 3, \y + \dy);

  \draw (6, \y) rectangle (6.5, \y + \dy);
  \draw (6.5, \y) rectangle (7, \y + \dy);
  \draw (7, \y) rectangle (7.5, \y + \dy);
  \draw (7.5, \y) rectangle (9, \y + \dy);
  \draw (8, \y) rectangle (8.5, \y + \dy);
  \draw (8.5, \y) rectangle (9, \y + \dy);
%  \fill[white] (6 + 0.1, \y + 0.7 * \dy) rectangle (9 - 0.1, \y + 0.3 * \dy);
%  \fill[pattern color=red, pattern=north west lines] (8, \y) rectangle (8.5, \y + \dy);

  \draw (9, \y) rectangle (10.5, \y + \dy);
  \draw (10.5, \y) rectangle (12, \y + \dy);
  \draw (12, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (9 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 11 * 0.5/3}
  
  \draw (26 * 0.5 / 3, \y) rectangle (27 * 0.5 / 3, \y + \dy);
  \draw (27 * 0.5 / 3, \y) rectangle (28 * 0.5 / 3, \y + \dy);
  \draw (28 * 0.5 / 3, \y) rectangle (29 * 0.5 / 3, \y + \dy);
  \draw (29 * 0.5 / 3, \y) rectangle (30 * 0.5 / 3, \y + \dy);
  \draw (30 * 0.5 / 3, \y) rectangle (31 * 0.5 / 3, \y + \dy);
  \draw (31 * 0.5 / 3, \y) rectangle (32 * 0.5 / 3, \y + \dy);
  \draw (32 * 0.5 / 3, \y) rectangle (33 * 0.5 / 3, \y + \dy);
  \draw (33 * 0.5 / 3, \y) rectangle (34 * 0.5 / 3, \y + \dy);
  \draw (34 * 0.5 / 3, \y) rectangle (35 * 0.5 / 3, \y + \dy);
  \draw (35 * 0.5 / 3, \y) rectangle (36 * 0.5 / 3, \y + \dy);

  \draw (6, \y) rectangle (6.5, \y + \dy);
  \draw (6.5, \y) rectangle (7, \y + \dy);
  \draw (7, \y) rectangle (7.5, \y + \dy);
  \draw (7.5, \y) rectangle (9, \y + \dy);
  \draw (8, \y) rectangle (8.5, \y + \dy);
  \draw (8.5, \y) rectangle (9, \y + \dy);
%  \fill[white] (6 + 0.1, \y + 0.7 * \dy) rectangle (9 - 0.1, \y + 0.3 * \dy);
%  \fill[pattern color=red, pattern=north west lines] (8, \y) rectangle (8.5, \y + \dy);

  \draw (9, \y) rectangle (10.5, \y + \dy);
  \draw (10.5, \y) rectangle (12, \y + \dy);
  \draw (12, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (9 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 12 * 0.5/3}
  
  \draw (29 * 0.5 / 3, \y) rectangle (30 * 0.5 / 3, \y + \dy);
  \draw (30 * 0.5 / 3, \y) rectangle (31 * 0.5 / 3, \y + \dy);
  \draw (31 * 0.5 / 3, \y) rectangle (32 * 0.5 / 3, \y + \dy);
  \draw (32 * 0.5 / 3, \y) rectangle (33 * 0.5 / 3, \y + \dy);
  \draw (33 * 0.5 / 3, \y) rectangle (34 * 0.5 / 3, \y + \dy);
  \draw (34 * 0.5 / 3, \y) rectangle (35 * 0.5 / 3, \y + \dy);
  \draw (35 * 0.5 / 3, \y) rectangle (36 * 0.5 / 3, \y + \dy);

  \draw (6, \y) rectangle (6.5, \y + \dy);
  \draw (6.5, \y) rectangle (7, \y + \dy);
  \draw (7, \y) rectangle (7.5, \y + \dy);
  \draw (7.5, \y) rectangle (9, \y + \dy);
  \draw (8, \y) rectangle (8.5, \y + \dy);
  \draw (8.5, \y) rectangle (9, \y + \dy);
%  \fill[white] (6 + 0.1, \y + 0.7 * \dy) rectangle (9 - 0.1, \y + 0.3 * \dy);
%  \fill[pattern color=red, pattern=north west lines] (8, \y) rectangle (8.5, \y + \dy);

  \draw (9, \y) rectangle (10.5, \y + \dy);
  \draw (10.5, \y) rectangle (12, \y + \dy);
  \draw (12, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (9 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 13 * 0.5/3}

  \draw (38 * 0.5 / 3, \y) rectangle (39 * 0.5 / 3, \y + \dy);
  \draw (39 * 0.5 / 3, \y) rectangle (40 * 0.5 / 3, \y + \dy);
  \draw (40 * 0.5 / 3, \y) rectangle (41 * 0.5 / 3, \y + \dy);
  \draw (41 * 0.5 / 3, \y) rectangle (42 * 0.5 / 3, \y + \dy);
  \draw (42 * 0.5 / 3, \y) rectangle (43 * 0.5 / 3, \y + \dy);
  \draw (43 * 0.5 / 3, \y) rectangle (44 * 0.5 / 3, \y + \dy);
  \draw (44 * 0.5 / 3, \y) rectangle (45 * 0.5 / 3, \y + \dy);

  \draw (7.5, \y) rectangle (8, \y + \dy);
  \draw (8, \y) rectangle (8.5, \y + \dy);
  \draw (8.5, \y) rectangle (9, \y + \dy);
%  \fill[white] (7.5 + 0.1, \y + 0.7 * \dy) rectangle (9 - 0.1, \y + 0.3 * \dy);
%  \fill[pattern color=red, pattern=north west lines] (8, \y) rectangle (8.5, \y + \dy);

  \draw (9, \y) rectangle (10.5, \y + \dy);
  \draw (10.5, \y) rectangle (12, \y + \dy);
  \draw (12, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (9 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 14 * 0.5/3}

  \draw (43 * 0.5 / 3, \y) rectangle (44 * 0.5 / 3, \y + \dy);
  \draw (44 * 0.5 / 3, \y) rectangle (45 * 0.5 / 3, \y + \dy);
  \draw (45 * 0.5 / 3, \y) rectangle (46 * 0.5 / 3, \y + \dy);
  \draw (46 * 0.5 / 3, \y) rectangle (47 * 0.5 / 3, \y + \dy);
  \draw (47 * 0.5 / 3, \y) rectangle (48 * 0.5 / 3, \y + \dy);
  \draw (48 * 0.5 / 3, \y) rectangle (49 * 0.5 / 3, \y + \dy);
  \draw (49 * 0.5 / 3, \y) rectangle (50 * 0.5 / 3, \y + \dy);
  \draw (50 * 0.5 / 3, \y) rectangle (51 * 0.5 / 3, \y + \dy);
  \draw (51 * 0.5 / 3, \y) rectangle (52 * 0.5 / 3, \y + \dy);
  \draw (52 * 0.5 / 3, \y) rectangle (53 * 0.5 / 3, \y + \dy);
  \draw (53 * 0.5 / 3, \y) rectangle (54 * 0.5 / 3, \y + \dy);

%  \fill[white] (7.5 + 0.1, \y + 0.7 * \dy) rectangle (9 - 0.1, \y + 0.3 * \dy);
%  \fill[pattern color=red, pattern=north west lines] (8, \y) rectangle (8.5, \y + \dy);

  \draw (9, \y) rectangle (9.5, \y + \dy);
  \draw (9.5, \y) rectangle (10, \y + \dy);
  \draw (10, \y) rectangle (10.5, \y + \dy);
  \draw (10.5, \y) rectangle (11, \y + \dy);
  \draw (11, \y) rectangle (11.5, \y + \dy);
  \draw (11.5, \y) rectangle (12, \y + \dy);
  \draw (12, \y) rectangle (12.5, \y + \dy);
  \draw (12.5, \y) rectangle (13, \y + \dy);
  \draw (13, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (9 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 15 * 0.5/3}

  \draw (47 * 0.5 / 3, \y) rectangle (48 * 0.5 / 3, \y + \dy);
  \draw (48 * 0.5 / 3, \y) rectangle (49 * 0.5 / 3, \y + \dy);
  \draw (49 * 0.5 / 3, \y) rectangle (50 * 0.5 / 3, \y + \dy);
  \draw (50 * 0.5 / 3, \y) rectangle (51 * 0.5 / 3, \y + \dy);
  \draw (51 * 0.5 / 3, \y) rectangle (52 * 0.5 / 3, \y + \dy);
  \draw (52 * 0.5 / 3, \y) rectangle (53 * 0.5 / 3, \y + \dy);
  \draw (53 * 0.5 / 3, \y) rectangle (54 * 0.5 / 3, \y + \dy);
%  \fill[pattern color=red, pattern=north west lines] (8, \y) rectangle (8.5, \y + \dy);

  \draw (9, \y) rectangle (9.5, \y + \dy);
  \draw (9.5, \y) rectangle (10, \y + \dy);
  \draw (10, \y) rectangle (10.5, \y + \dy);
  \draw (10.5, \y) rectangle (11, \y + \dy);
  \draw (11, \y) rectangle (11.5, \y + \dy);
  \draw (11.5, \y) rectangle (12, \y + \dy);
  \draw (12, \y) rectangle (12.5, \y + \dy);
  \draw (12.5, \y) rectangle (13, \y + \dy);
  \draw (13, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (9 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 16 * 0.5/3}

  \draw (53 * 0.5 / 3, \y) rectangle (54 * 0.5 / 3, \y + \dy);
  \draw (54 * 0.5 / 3, \y) rectangle (55 * 0.5 / 3, \y + \dy);
  \draw (55 * 0.5 / 3, \y) rectangle (56 * 0.5 / 3, \y + \dy);
  \draw (56 * 0.5 / 3, \y) rectangle (57 * 0.5 / 3, \y + \dy);
  \draw (57 * 0.5 / 3, \y) rectangle (58 * 0.5 / 3, \y + \dy);
  \draw (58 * 0.5 / 3, \y) rectangle (59 * 0.5 / 3, \y + \dy);
  \draw (59 * 0.5 / 3, \y) rectangle (60 * 0.5 / 3, \y + \dy);
  \draw (60 * 0.5 / 3, \y) rectangle (61 * 0.5 / 3, \y + \dy);
  \draw (61 * 0.5 / 3, \y) rectangle (62 * 0.5 / 3, \y + \dy);
  \draw (62 * 0.5 / 3, \y) rectangle (63 * 0.5 / 3, \y + \dy);
  
  \draw (10.5, \y) rectangle (11, \y + \dy);
  \draw (11, \y) rectangle (11.5, \y + \dy);
  \draw (11.5, \y) rectangle (12, \y + \dy);
  \draw (12, \y) rectangle (12.5, \y + \dy);
  \draw (12.5, \y) rectangle (13, \y + \dy);
  \draw (13, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (9 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 17 * 0.5/3}
  
  \draw (53 * 0.5 / 3, \y) rectangle (54 * 0.5 / 3, \y + \dy);
  \draw (54 * 0.5 / 3, \y) rectangle (55 * 0.5 / 3, \y + \dy);
  \draw (55 * 0.5 / 3, \y) rectangle (56 * 0.5 / 3, \y + \dy);
  \draw (56 * 0.5 / 3, \y) rectangle (57 * 0.5 / 3, \y + \dy);
  \draw (57 * 0.5 / 3, \y) rectangle (58 * 0.5 / 3, \y + \dy);
  \draw (58 * 0.5 / 3, \y) rectangle (59 * 0.5 / 3, \y + \dy);
  \draw (59 * 0.5 / 3, \y) rectangle (60 * 0.5 / 3, \y + \dy);
  \draw (60 * 0.5 / 3, \y) rectangle (61 * 0.5 / 3, \y + \dy);
  \draw (61 * 0.5 / 3, \y) rectangle (62 * 0.5 / 3, \y + \dy);
  \draw (62 * 0.5 / 3, \y) rectangle (63 * 0.5 / 3, \y + \dy);

  \draw (10.5, \y) rectangle (11, \y + \dy);
  \draw (11, \y) rectangle (11.5, \y + \dy);
  \draw (11.5, \y) rectangle (12, \y + \dy);

  \draw (12, \y) rectangle (12.5, \y + \dy);
  \draw (12.5, \y) rectangle (13, \y + \dy);
  \draw (13, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (10.5 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

  \def\y{10 - 18 * 0.5/3}
  
  \draw (58 * 0.5 / 3, \y) rectangle (59 * 0.5 / 3, \y + \dy);
  \draw (59 * 0.5 / 3, \y) rectangle (60 * 0.5 / 3, \y + \dy);
  \draw (60 * 0.5 / 3, \y) rectangle (61 * 0.5 / 3, \y + \dy);
  \draw (61 * 0.5 / 3, \y) rectangle (62 * 0.5 / 3, \y + \dy);
  \draw (62 * 0.5 / 3, \y) rectangle (63 * 0.5 / 3, \y + \dy);

  \draw (10.5, \y) rectangle (11, \y + \dy);
  \draw (11, \y) rectangle (11.5, \y + \dy);
  \draw (11.5, \y) rectangle (12, \y + \dy);
%  \fill[white] (10.5 + 0.1, \y + 0.7 * \dy) rectangle (12 - 0.1, \y + 0.3 * \dy);

  \draw (12, \y) rectangle (12.5, \y + \dy);
  \draw (12.5, \y) rectangle (13, \y + \dy);
  \draw (13, \y) rectangle (13.5, \y + \dy);
%  \fill[white] (12 + 0.1, \y + 0.7 * \dy) rectangle (13.5 - 0.1, \y + 0.3 * \dy);

%  \draw[thick, red] (1.25, 7.2 + 0.5 * \dy) rectangle (8.25, 3.6 + 0.5 * \dy);
%  \draw[thick, decorate, decoration={calligraphic brace, amplitude=5pt}, yshift=-10pt] (8.25, 3.6 + 0.5 * \dy) to node[pos=0.5, below, yshift=-5pt] {maximum allowed deficit} (1.25, 3.6 + 0.5 * \dy);
  
